Coordinate-View Confusability Graphs and Matroid Rank Certificates

A coordinate-view presentation specifies a large confusability graph by coordinates rather than by an edge list. The problem is to certify zero-error recovery and Shannon capacity from the succinct presentation, before the exponentially large graph is materialized. For affine presentations over $\mathbb F_q$, Gaussian elimination gives a polynomial-time rank upper certificate from $O(rd\log q+Ld)$ input bits for a graph with $q^r$ vertices. Exactness of that certificate is equivalent to positivity of a Grassmannian avoidance count $N_{t^*}$. Positivity of $N_k$ is NP-complete for every fixed $k$, already over $\mathbb F_2$, while the ambient-rank parameter gives a fixed-parameter algorithm. The rank-one reduction is parsimonious for $\#SAT$. For arbitrary $t$, the finite decoder for $N_t$ reads the signed rank profile of the represented forbidden-point matroid; the kernel-intersection lattice alone does not determine the count. On the positive side, kernel sections give the exact formula $\Theta(G)=\log\alpha(G)=\min_{S\in\mathcal V}t(S)\log q$, with a projection-equality matrix optimal for Haemers minrank. A finite-field blocking theorem gives exactness when $q\ge L$, and Reed-Solomon/MDS codes give exact all-$k$-view families beyond that regime. Full-tuple coordinate-view graphs also have a polynomial-time cofinal-antichain normal form; transitive confusability is exactly intersection closure.

==> content/assumption_ledger_auto.tex <==
% Auto-generated by scripts/build_papers.py. Do not edit manually.
% Generated: 2026-07-01T13:46:14.023473
\subsection{Assumption Ledger (Auto)}
\paragraph{Source files.}
\begin{itemize}
\item \nolinkurl{Ssot/HandleAliases.lean}
\end{itemize}
\paragraph{Assumption bundles and fields.}
\begin{itemize}
\item (No assumption bundles parsed.)
\end{itemize}
\paragraph{Conditional closure handles.}
\begin{itemize}
\item (No conditional theorem handles parsed.)
\end{itemize}
\paragraph{First-principles Bayes derivation handles.}
\begin{itemize}
\item (No Bayes-derivation theorem handles found.)
\end{itemize}
\paragraph{Compact Bayes handle IDs.}
\begin{itemize}
\item (No compact Bayes alias IDs found.)
\end{itemize}


==> content/proof_hardness_index_auto.tex <==
% Auto-generated by scripts/build_papers.py. Do not edit manually.
% Generated: 2026-07-01T13:46:15.122360
% Manuscript: paper2_it
\begingroup
\scriptsize
\sloppy
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}
\begin{longtable}{@{}>{\raggedright\arraybackslash}m{0.19\linewidth}>{\raggedright\arraybackslash}m{0.13\linewidth}>{\raggedright\arraybackslash}m{0.26\linewidth}>{\raggedright\arraybackslash}m{0.38\linewidth}@{}}
\toprule
\textbf{Manuscript handle} & \textbf{Hardness profile} & \textbf{Regime tags} & \textbf{Lean support} \\
\midrule
\endfirsthead
\toprule
\textbf{Manuscript handle} & \textbf{Hardness profile} & \textbf{Regime tags} & \textbf{Lean support} \\
\midrule
\endhead
\endfoot
\bottomrule
\endlastfoot
\nolinkurl{cor:graphic-matroid-rank-sieve-counting-hard} & \nolinkurl{#P-hard} & - & \LH{GCB3}, \LH{GCB4}, \LH{GCB5}, \LH{GCB6}, \LH{GCB7}, \LH{GCB8}, \LH{GCB9}, \LH{GCB10}, \LH{GCB11}, \LH{GCB12}, \LH{GCB13}, \LH{GCB14}, \LH{GCB15}, \LH{GCB16}, \LH{GCB17}, \LH{GCB18}, \LH{GCB19}, \LH{GCB20}, \LH{GCB21}, \LH{GCB22}, \LH{GCB23}, \LH{GCB24}, \LH{GCB25}, \LH{GCB26}, \LH{GCB27}, \LH{GCB28}, \LH{GCB29}, \LH{GCB30}, \LH{GCB31}, \LH{GCB32}, \LH{GCB33}, \LH{GCB34}, \LH{GCB35}, \LH{GCB36}, \LH{GCB37}, \LH{GCB38}, \LH{GCB39}, \LH{GCB40}, \LH{GCB41}, \LH{GCB42}, \LH{GCR121}, \LH{GCR122}, \LH{GCR123}, \LH{GCR124}, \LH{GCR125} \\
\midrule
\nolinkurl{cor:rank-one-avoidance-counting-hard} & \nolinkurl{#P-hard} & - & \LH{KSH14}, \LH{KSH15} \\
\midrule
\nolinkurl{cor:fixed-rank-kernel-section-np-complete} & \nolinkurl{NP-complete} & - & \LH{AKS35}, \LH{KSH1}, \LH{KSH2}, \LH{KSH3}, \LH{KSH4}, \LH{KSH5}, \LH{KSH9}, \LH{KSH10}, \LH{KSH11} \\
\midrule
\nolinkurl{cor:grassmannian-avoidance-positivity-np-complete} & \nolinkurl{NP-complete} & - & \LH{ABD10}, \LH{AKS35}, \LH{KSH1}, \LH{KSH2}, \LH{KSH3}, \LH{KSH4}, \LH{KSH5}, \LH{KSH9}, \LH{KSH10}, \LH{KSH11} \\
\midrule
\nolinkurl{cor:rank-one-nonlinear-section-np-hard} & \nolinkurl{NP-complete} & - & \LH{KSH6}, \LH{KSH7}, \LH{KSH8}, \LH{KSH12}, \LH{KSH13} \\
\midrule
\nolinkurl{thm:rank-one-kernel-section-np-hard} & \nolinkurl{NP-complete} & - & \LH{KSH1}, \LH{KSH2}, \LH{KSH3}, \LH{KSH4}, \LH{KSH5}, \LH{KSH9}, \LH{KSH10}, \LH{KSH11} \\
\midrule
\nolinkurl{thm:field-size-exactness} & \nolinkurl{P/exact for q>=L} & - & \LH{AFM24}, \LH{AKS6}, \LH{AKS7}, \LH{AKS8}, \LH{AKS9}, \LH{AKS17}, \LH{AKS18} \\
\midrule
\nolinkurl{lem:finite-union-subspace-avoidance} & \nolinkurl{finite-field covering bound} & - & \LH{AKS6}, \LH{AKS7}, \LH{AKS17}, \LH{AKS18} \\
\midrule
\nolinkurl{thm:fixed-lattice-sat-spine} & \nolinkurl{fixed-lattice SAT/#SAT} & - & \LH{SCB979}, \LH{SCB980}, \LH{SCB981}, \LH{SCB982}, \LH{SCB983}, \LH{SCB984}, \LH{SCB985}, \LH{SCB986}, \LH{SCB987}, \LH{SCB988}, \LH{SCB989}, \LH{SCB990}, \LH{SCB991}, \LH{SCB992}, \LH{SCB993}, \LH{SCB994}, \LH{SCB995}, \LH{SCB996}, \LH{SCB997}, \LH{SCB998}, \LH{SCB999}, \LH{SCB1000}, \LH{SCB1001}, \LH{SCB1002}, \LH{SCB1003}, \LH{SCB1004}, \LH{SCB1005}, \LH{SCB1006}, \LH{SCB1007}, \LH{SCB1008}, \LH{SCB1009}, \LH{SCB1010}, \LH{SCB1011}, \LH{SCB1012}, \LH{SCB1013} \\
\midrule
\nolinkurl{cor:arrangement-support-profile} & \nolinkurl{structural/exact} & - & \LH{AKS36}, \LH{AKS37}, \LH{AKS38} \\
\midrule
\nolinkurl{cor:haemers-optimal-kernel-section} & \nolinkurl{structural/exact} & - & \LH{AKS1}, \LH{AKS2}, \LH{AKS3}, \LH{AKS4}, \LH{AKS5}, \LH{MFT95} \\
\midrule
\nolinkurl{cor:kernel-section-direct-sum} & \nolinkurl{structural/exact} & - & \LH{AFM17}, \LH{AFM18}, \LH{AFM19}, \LH{AKS1}, \LH{AKS2}, \LH{AKS3}, \LH{AKS4}, \LH{AKS5}, \LH{MFT25}, \LH{MFT26} \\
\midrule
\nolinkurl{cor:kernel-section-no-gap} & \nolinkurl{structural/exact} & - & \LH{AKS32} \\
\midrule
\nolinkurl{cor:rank-additivity-block} & \nolinkurl{structural/exact} & - & \LH{AFM17} \\
\midrule
\nolinkurl{cor:subcode-distance-boundary} & \nolinkurl{structural/exact} & - & \LH{AKS34} \\
\midrule
\nolinkurl{lem:common-core-lift} & \nolinkurl{structural/exact} & - & \LH{ABD28}, \LH{ABD29}, \LH{ABD30}, \LH{ABD31}, \LH{ABD32}, \LH{ABD33}, \LH{ABD34}, \LH{ABD35}, \LH{ABD42}, \LH{ABD48}, \LH{ABD49}, \LH{ABD50}, \LH{ABD51}, \LH{ABD52}, \LH{ABD53}, \LH{ABD54}, \LH{ABD55}, \LH{ABD56} \\
\midrule
\nolinkurl{prop:affine-kernel-sum-transitivity} & \nolinkurl{structural/exact} & - & \LH{AKS22}, \LH{AKS23}, \LH{AKS24}, \LH{AKS25}, \LH{AKS26}, \LH{AKS27}, \LH{AKS28}, \LH{AKS29}, \LH{AKS30}, \LH{AKS31} \\
\midrule
\nolinkurl{prop:agreement-family-complete-invariant} & \nolinkurl{structural/exact} & - & \LH{MFT202} \\
\midrule
\nolinkurl{prop:all-k-view-hamming-threshold} & \nolinkurl{structural/exact} & - & \LH{MFT102}, \LH{MFT103}, \LH{MFT104}, \LH{MFT105}, \LH{MFT106} \\
\midrule
\nolinkurl{prop:block-composition-strong-product} & \nolinkurl{structural/exact} & - & \LH{MFT25}, \LH{MFT26} \\
\midrule
\nolinkurl{prop:hamming-endpoint-family} & \nolinkurl{structural/exact} & - & \LH{AKS19} \\
\midrule
\nolinkurl{prop:matroid-direct-sum-block} & \nolinkurl{structural/exact} & - & \LH{AFM18}, \LH{AFM19} \\
\midrule
\nolinkurl{prop:subfamily-certificate-hierarchy} & \nolinkurl{structural/exact} & - & \LH{MFT92}, \LH{MFT93}, \LH{MFT94} \\
\midrule
\nolinkurl{prop:support-hitting-sections} & \nolinkurl{structural/exact} & - & \LH{AKS20}, \LH{AKS21}, \LH{AKS36}, \LH{AKS37}, \LH{AKS38} \\
\midrule
\nolinkurl{prop:view-fiber-clique-sizes} & \nolinkurl{structural/exact} & - & \LH{AFM6}, \LH{AFM7}, \LH{AFM8}, \LH{AFM9}, \LH{AFM10}, \LH{AFM11}, \LH{AFM12}, \LH{MFT86} \\
\midrule
\nolinkurl{thm:affine-fact-matroid} & \nolinkurl{structural/exact} & - & \LH{AFM1}, \LH{AFM2}, \LH{AFM3}, \LH{AFM4}, \LH{AFM5}, \LH{AFM20}, \LH{AFM21}, \LH{AFM22} \\
\midrule
\nolinkurl{thm:intersection-closure} & \nolinkurl{structural/exact} & - & \LH{MFT139}, \LH{MFT140}, \LH{MFT141}, \LH{MFT142}, \LH{MFT143}, \LH{MFT144}, \LH{MFT145}, \LH{MFT146}, \LH{MFT147}, \LH{MFT148}, \LH{MFT149}, \LH{MFT150} \\
\midrule
\nolinkurl{thm:kernel-section-exactness} & \nolinkurl{structural/exact} & - & \LH{AKS1}, \LH{AKS2}, \LH{AKS3}, \LH{AKS4}, \LH{AKS5} \\
\midrule
\nolinkurl{thm:matroid-capacity-bounds} & \nolinkurl{structural/exact} & - & \LH{AFM6}, \LH{AFM7}, \LH{AFM8}, \LH{AFM9}, \LH{AFM10}, \LH{AFM11}, \LH{AFM12} \\
\midrule
\nolinkurl{thm:pair-injective} & \nolinkurl{structural/exact} & - & \LH{OBS1}, \LH{OBS2} \\
\midrule
\nolinkurl{thm:signed-profile-compression} & \nolinkurl{structural/exact} & - & \LH{ABD21}, \LH{ABD22}, \LH{ABD23}, \LH{ABD79}, \LH{ABD80}, \LH{ABD81}, \LH{ABD82}, \LH{ABD83}, \LH{ABD84}, \LH{ABD85}, \LH{ABD86}, \LH{ABD87}, \LH{ABD88}, \LH{ABD89}, \LH{ABD90}, \LH{ABD91}, \LH{SPB240}, \LH{SPB241}, \LH{SPB242}, \LH{SPB243}, \LH{SPB244}, \LH{SPB245}, \LH{SPB288}, \LH{SPB289}, \LH{SPB379}, \LH{SPB380}, \LH{SPB381}, \LH{SPB382}, \LH{SPB383} \\
\bottomrule
\end{longtable}
\endgroup

\noindent\textit{Auto summary: indexed 31 claims by hardness profile (#P-hard=2; NP-complete=4; P/exact for q>=L=1; finite-field covering bound=1; fixed-lattice SAT/#SAT=1; structural/exact=22).}


==> paper_title_auto.tex <==
% Auto-generated by scripts/build_papers.py. Canonical manuscript title.
\providecommand{\PaperTitleAuto}{Coordinate-View Confusability Graphs and Matroid Rank Certificates}

